Testing for Outliers with Conformal p-values

This paper studies the construction of p-values for nonparametric outlier detection, taking a multiple-testing perspective. The goal is to test whether new independent samples belong to the same distribution as a reference data set or are outliers. We propose a solution based on conformal inference, a broadly applicable framework which yields p-values that are marginally valid but mutually dependent for different test points. We prove these p-values are positively dependent and enable exact false discovery rate control, although in a relatively weak marginal sense. We then introduce a new method to compute p-values that are both valid conditionally on the training data and independent of each other for different test points; this paves the way to stronger type-I error guarantees. Our results depart from classical conformal inference as we leverage concentration inequalities rather than combinatorial arguments to establish our finite-sample guarantees. Furthermore, our techniques also yield a uniform confidence bound for the false positive rate of any outlier detection algorithm, as a function of the threshold applied to its raw statistics. Finally, the relevance of our results is demonstrated by numerical experiments on real and simulated data.

==> tables_new/data_bh_small.tex <==
\begin{table}[!htb]

\caption{Outlier detection performance on different data sets, using alternative methods for calibrating conformal p-values. 
The FDR and power diagnostics are defined conditional on the training and calibration data, as explained in Section~\ref{sec:exp-setup}. The nominal marginal FDR level is 0.2. Empirical FDR values larger than the nominal level are colored in orange; values at least one standard deviation above it are colored in red. \label{tab:data-bh-storey}}
\centering
\fontsize{10}{12}\selectfont
\begin{tabular}[t]{lllllllll}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{4}{c}{FDR} & \multicolumn{4}{c}{Power} \\
\cmidrule(l{3pt}r{3pt}){2-5} \cmidrule(l{3pt}r{3pt}){6-9}
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Mean} & \multicolumn{2}{c}{90th percentile} & \multicolumn{2}{c}{Mean} & \multicolumn{2}{c}{90-th quantile} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7} \cmidrule(l{3pt}r{3pt}){8-9}
Dataset & Marg. & Cond. & Marg. & Cond. & Marg. & Cond. & Marg. & Cond.\\
\midrule
ALOI & 0.032 & 0.002 & 0.08 & 0 & 0 & 0 & 0 & 0\\
Cover & 0.089 & 0.03 & \textcolor{red}{0.285} & 0.083 & 0.01 & 0.005 & 0.035 & 0.013\\
Credit card & 0.173 & 0.146 & \textcolor{orange}{0.212} & 0.186 & 0.642 & 0.57 & 0.763 & 0.712\\
KDDCup99 & 0.174 & 0.124 & \textcolor{orange}{0.209} & 0.159 & 0.736 & 0.673 & 0.796 & 0.745\\
Mammography & 0.167 & 0.054 & \textcolor{red}{0.269} & 0.169 & 0.156 & 0.058 & 0.305 & 0.217\\
\addlinespace
Digits & 0.182 & 0.054 & \textcolor{red}{0.248} & 0.174 & 0.357 & 0.099 & 0.59 & 0.326\\
Shuttle & 0.178 & 0.149 & \textcolor{orange}{0.212} & 0.187 & 0.98 & 0.979 & 0.983 & 0.983\\
\bottomrule
\end{tabular}
\end{table}


==> tables_new/data_global_bh_small.tex <==
\begin{table}

\caption{Outlier batch detection performance on different data sets, using alternative methods for calibrating conformal p-values. The nominal FDR level is 0.1. Other details are as in Table~\ref{tab:data-bh-storey}. \label{tab:data-global-storey}}
\centering
\fontsize{10}{12}\selectfont
\begin{tabular}[t]{lllllllll}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{4}{c}{FDR} & \multicolumn{4}{c}{Power} \\
\cmidrule(l{3pt}r{3pt}){2-5} \cmidrule(l{3pt}r{3pt}){6-9}
\multicolumn{1}{c}{ } & \multicolumn{2}{c}{Mean} & \multicolumn{2}{c}{90-th quantile} & \multicolumn{2}{c}{Mean} & \multicolumn{2}{c}{90-th quantile} \\
\cmidrule(l{3pt}r{3pt}){2-3} \cmidrule(l{3pt}r{3pt}){4-5} \cmidrule(l{3pt}r{3pt}){6-7} \cmidrule(l{3pt}r{3pt}){8-9}
Data set & Marg. & Cond. & Marg. & Cond. & Marg. & Cond. & Marg. & Cond.\\
\midrule
ALOI & 0.067 & 0.021 & \textcolor{red}{0.191} & 0.096 & 0.001 & 0 & 0.004 & 0.002\\
Cover & 0.072 & 0.046 & \textcolor{red}{0.143} & \textcolor{orange}{0.111} & 0.168 & 0.126 & 0.309 & 0.234\\
Credit card & 0.077 & 0.056 & \textcolor{orange}{0.116} & 0.087 & 0.98 & 0.973 & 0.992 & 0.986\\
KDDCup99 & 0.08 & 0.043 & \textcolor{orange}{0.126} & 0.079 & 0.999 & 0.998 & 1 & 1\\
Mammography & 0.069 & 0.018 & \textcolor{orange}{0.111} & 0.044 & 0.606 & 0.376 & 0.736 & 0.56\\
Digits & 0.075 & 0.019 & \textcolor{orange}{0.118} & 0.037 & 0.966 & 0.851 & 0.994 & 0.952\\
Shuttle & 0.084 & 0.046 & \textcolor{red}{0.131} & 0.084 & 1 & 1 & 1 & 1\\
\bottomrule
\end{tabular}
\end{table}

